A Survey on Product Operators in Abstract Interpretation

The aim of this paper is to provide a general overview of the product operators introduced in the literature as a tool to enhance the analysis accuracy in the Abstract Interpretation framework. In particular we focus on the Cartesian and reduced products, as well as on the reduced cardinal power, an under-used technique whose features deserve to be stressed for their potential impact in practical applications.

==> eptcsdata.tex <==
\providecommand{\firstpage}{325}
\providecommand{\publicationstatus}{A. Banerjee, O. Danvy, K.-G. Doh, J. Hatcliff (Eds):\\
David A. Schmidt's 60th Birthday Festschrift\\
EPTCS 129, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.129.19}{10.4204/EPTCS.129.19}}
\pdfoutput=1

